FedMPDD: Communication-Efficient Federated Learning with Privacy Preservation Attributes via Projected Directional Derivative

This paper introduces \texttt{FedMPDD} (\textbf{Fed}erated Learning via \textbf{M}ulti-\textbf{P}rojected \textbf{D}irectional \textbf{D}erivatives), a novel algorithm that simultaneously optimizes bandwidth utilization and enhances privacy in Federated Learning. The core idea of \texttt{FedMPDD} is to encode each client's high-dimensional gradient by computing its directional derivatives along multiple random vectors. This compresses the gradient into a much smaller message, significantly reducing uplink communication costs from $\mathcal{O}(d)$ to $\mathcal{O}(m)$, where $m \ll d$. The server then decodes the aggregated information by projecting it back onto the same random vectors. Our key insight is that averaging multiple projections overcomes the dimension-dependent convergence limitations of a single projection. We provide a rigorous theoretical analysis, establishing that \texttt{FedMPDD} converges at a rate of $\mathcal{O}(1/\sqrt{K})$, matching the performance of FedSGD. Furthermore, we demonstrate that our method provides some inherent privacy against gradient inversion attacks due to the geometric properties of low-rank projections, offering a tunable privacy-utility trade-off controlled by the number of projections. Extensive experiments on benchmark datasets validate our theory and demonstrates our results.

==> intro.tex <==
\section{Introduction}\label{sec::Intro}
Federated Learning (FL) is a foundational paradigm for collaboratively training models across $N$ edge devices by leveraging their local computational resources~\cite{mcmahan2017communication, kairouz2021advances, chen2019deep, wang2023model}\margin{add fed LQR references also}. FL seeks to solve the distributed optimization problem:
\begin{equation}\label{eq::opt_prob}
\text{minimize}_{\vect{x}\in\mathbb{R}^d}~~ f(\vect{x}) = \frac{1}{N} \sum\nolimits_{i=1}^N f_i(\vect{x}).
\end{equation}
Here, $f_i:\mathbb{R}^d\to\mathbb{R}$  is the local objective (loss) function of client $i$, and $f:\mathbb{R}^d\to\mathbb{R}$  is the global objective. Lacking central access to local objectives, FL iteratively communicates between a server and a client subset $\mathcal{A}_k$ ( $|\mathcal{A}_k|=\beta N$, where \( \beta \in (0, 1] \) denotes the client participation rate). In each round $k$, the server sends out the global model $\vect{x}_k$. Selected clients compute local updates (e.g., mini-batch gradients $\vect{g}_i(\vect{x}_k)$) and transmit them to the server. The server aggregates these gradients by averaging: $\vect{g}(\vect{x}_k) = \frac{1}{\beta N} \sum_{i \in \mathcal{A}_k} \vect{g}_i(\vect{x}_k)$, and updates the global model: $\vect{x}_{k+1} = \vect{x}_k - \eta ~\vect{g}(\vect{x}_k)$, as in \texttt{FedSGD}~\cite{mcmahan2017communication}, where  $\eta$ is a suitable learning rate.

\medskip

 A key bottleneck in FL algorithms like \texttt{FedSGD} is the substantial uplink communication overhead from transmitting $d$-dimensional gradients $\vect{g}_i(\vect{x}_k)$ from clients to the server, requiring \(32d\) bits per client per round, assuming single-precision floating-point representation (32 bits per value). For instance, a ResNet-18 model ($\sim 11 \times 10^6$ parameters) necessitates approximately $42$MB transmission per client per round. This high cost severely impacts efficiency in bandwidth-constrained real-world deployments~\cite{chen2021communication, niknam2020federated, shahid2021communication, li2020federated}. Strategies to reduce FL communication volume or frequency fall into three main classes: \emph{model compression}, \emph{local computation with client selection}, and \emph{gradient compression}. Model compression reduces global model size, for example, by using smaller models with local representations~\cite{liang2020think}. Local computation and client selection decrease communication frequency or the number of clients per round through techniques like multiple local updates~\cite{stich2018local, mcmahan2017communication, karimireddy2020scaffold} and client subset selection~\cite{sattler2019robust, liang2020think}. Gradient compression reduces the size of transmitted gradients using methods like quantization~\cite{alistarh2017qsgd, horvoth2022natural, karimireddy2019error,shlezinger2020uveqfed, bernstein2018signsgd, reisizadeh2020fedpaq, suresh2017distributed}, sparsification~\cite{ivkin2019communication, lin2017deep}, and structured/sketched updates~\cite{konevcny2016federated, wang2020federated, azam2021recycling, han2024random, ivkin2019communication, cho2024heterogeneous, kuo2024federated, qi2024fdlora, yi2023pfedlora, lin2022personalized}.

\medskip
This paper proposes a novel framework that tackles the critical communication efficiency bottleneck to enable more practical and scalable deployment of FL in bandwidth-constrained environments. Unlike existing gradient compression techniques such as quantization, sparsification, or structured/sketched updates, our approach introduces a fundamentally new multiplicative encoding paradigm through the \emph{projected directional derivative} within the FL framework. Our algorithm follows the core structure of \texttt{FedSGD} but employs the \emph{projected directional derivative} $\hat{\vect{g}}_i(\vect{x}_k)=\vect{u}_{k,i}^\top\vect{g}_i(\vect{x}_k)\vect{u}_{k,i}$ (defined in~\eqref{def:proj}) instead of the stochastic gradient $\vect{g}_i(\vect{x}_k)$ to achieve dramatic communication reduction. We decompose the projected directional gradient into a scalar directional derivative 
$\vect{u}_{k,i}^\top \vect{g}_i(\vect{x}_k)$ computed locally by client $i$. 
Each client independently samples $\vect{u}_{k,i}$, then transmits only two scalars: 
the directional derivative $\vect{u}_{k,i}^\top \vect{g}_i(\vect{x}_k)$ and the random seed $r_{k,i}$ used to generate $\vect{u}_{k,i}$. 
On the server side, the received seed $r_{k,i}$ is used to reconstruct the identical $d$-dimensional vector $\vect{u}_{k,i}$, 
enabling the server to form the gradient estimator $\hat{\vect{g}}_{i}(\vect{x}_{k})$ without ever transmitting the full vector. The noisy gradient estimator from a single projected directional derivative can degrade performance. To address this, we propose our main algorithm \texttt{FedMPDD} (\textbf{Fed}erated Learning via \textbf{M}ulti-\textbf{P}rojected \textbf{D}irectional \textbf{D}erivatives), which introduces a principled multi-projection aggregation mechanism that averages $m$ projected directional derivatives to estimate the gradient and form our FL algorithm, leading to the following key contributions:
\begin{itemize}[leftmargin=10pt]
    \item \textbf{Significant Communication Reduction:} 
    \texttt{FedMPDD} dramatically reduces uplink communication from $O(d)$ to just $m + 1$ scalars per client per round ($O(m)$ bits, where $m \ll d$), achieving orders of magnitude reduction in communication overhead. For example, with $m=100$ projections on a ResNet-18 model ($d \approx 11 \times 10^6$), we reduce communication from $42$MB to approximately $0.4$KB per client per round, representing a $\sim 100,000\times$ reduction while maintaining competitive model performance.

    \item \textbf{Fast Convergence with Multi-Projection Averaging}: Unlike single-projection approaches that suffer from dimension-dependent convergence, \texttt{FedMPDD} achieves a convergence rate of $O(1/\sqrt{K})$ (Theorem~\ref{thm:main_2}), comparable to standard \texttt{FedSGD} baselines, through our novel multi-projection averaging mechanism. The parameter $m$ provides a tunable trade-off between communication cost and convergence speed, enabling flexible adaptation to varying bandwidth constraints.
    
    \item \textbf{Inherent Privacy Preservation as a Side Benefit:} 
    An interesting emergent property of our communication reduction scheme is that it naturally provides privacy protection against gradient inversion attacks (GIAs). The privacy guarantee arises from the rank-deficiency of the projection matrix $\frac{1}{m}\,\mat{U}_{k,i} \mat{U}_{k,i}^\top$, where $\mat{U}_{k,i}$ is the aggregate matrix of $\{\vect{u}_{k,i}^{(j)}\}_{j=1}^{m}$. This geometric nullspace property creates an underdetermined system that prevents unique gradient recovery, fundamentally different from additive noise methods like local differential privacy (LDP). Unlike LDP approaches, \texttt{FedMPDD} offers uniform privacy protection regardless of gradient magnitude without requiring additional noise injection that can degrade convergence (Remark~\ref{remark_bound}).
\end{itemize}

\medskip
While our primary focus is communication efficiency, it is worth noting the privacy context of FL. Although FL avoids direct data sharing by performing local training, recent studies have shown that a client's raw data can be reconstructed from its transmitted gradients~\cite{zhu2019deep, zhao2020idlg, huang2021evaluating, yin2021see, melis2019exploiting, li2022e2egi} via Gradient Inversion Attacks (GIAs). 
In GIAs within FL, a honest-but-curious server (or any adversary with the same level of server's global information) employs a deep neural network as an inversion model. This inversion network is trained to find input data that, when used to compute gradients, closely matches the gradients shared by legitimate clients, thereby revealing private information~\cite{yin2021comprehensive, geiping2020inverting, jere2020taxonomy, nasr2019comprehensive}. A common privacy preservation measure is via a local differential privacy (LDP) framework \cite{wei2020federated, truex2020ldp, zhao2020local, seif2020wireless}, where each client adds noise to its gradient before uploading it to the server.  By injecting noise locally, LDP enhances privacy protection without relying on a trusted aggregator. However, this approach introduces a fundamental trade-off between privacy and convergence~\cite{jere2020taxonomy}. In contrast, the privacy protection in \texttt{FedMPDD} emerges naturally from the communication reduction mechanism itself: the rank deficiency of $\vect{u}_{k, i}\vect{u}_{k, i}^\top$ in $\hat{\vect{g}}_i(\vect{x}_k)=\vect{u}_{k,i}^\top\vect{g}_i(\vect{x}_k)\vect{u}_{k,i}=\vect{u}_{k, i}\vect{u}_{k, i}^\top\vect{g}_i(\vect{x}_k)$ creates an underdetermined system that prevents unique gradient recovery, without requiring explicit noise addition or sacrificing the communication benefits.

\vspace{-6pt}
Extensive comparative theoretical analysis and empirical evaluations demonstrate \texttt{FedMPDD}'s superior communication efficiency and model performance, with the added advantage of inherent privacy preservation.




\textbf{Related Work.} 
Our method is fundamentally distinct from structured and sketched updates, which reduce communication by projecting data onto a \textit{fixed}, low-dimensional subspace. Structured updates, such as low-rank adaptation, use a pre-defined subspace for parameters \cite{hu2022lora, yi2023pfedlora, qi2024fdlora, zhang2018systematic, ullrich2017soft, bertsimas2023new, cho2024heterogeneous}. Similarly, sketched updates compress gradients using a shared random matrix, fixed at initialization, via techniques like projection matrices \cite{park2023regulated, azam2021recycling, guo2024low} or Count-Sketch \cite{ivkin2019communication, rothchild2020fetchsgd, haddadpour2020fedsketch, jiang2018sketchml}. These approaches rely on a static projection for all clients and rounds, with some variants incurring significant computational overhead to minimize reconstruction error in the fixed subspace \cite{lin2022personalized}. In contrast, our approach uses a \textit{dynamic} projection strategy based on multi-projected directional derivatives. We compute $\hat{g}_i(x_k) = (u_{k,i}^\top g_i(x_k)) u_{k,i}$, where the projection directions $u_{k,i}$ are randomly and independently sampled for each client $i$ at every round $k$. By averaging multiple projections ($m \ll d$), we overcome the rank-deficiency of a single direction and achieve $O(1/\sqrt{K})$ convergence while reducing communication to $O(m)$ bits. This dynamic multi-projection mechanism simultaneously provides dramatic communication reduction and, as an inherent by-product, privacy protection through the nullspace effect, representing a fundamental departure from methods reliant on fixed subspaces.

The \emph{projected directional derivative} has been explored in optimization, including balancing computational cost and memory in deep learning gradient calculations~\cite{fournier2023can, ren2022scaling, silver2021learning, baydin2022gradients} and in zeroth-order optimization~\cite{nesterov2017random}. To our knowledge, this is the first work to introduce the \emph{projected directional derivative} in FL, specifically through a novel multi-projection decomposition that addresses the dimension-dependent convergence limitations of single-projection methods while achieving substantial communication reduction. 

Regarding \emph{joint privacy preservation and communication management}, some communication management techniques offer privacy as a side benefit \cite{lang2023joint, agarwal2018cpsgd}. Amiri et al.~\cite{amiri2021compressive} combined differential privacy (DP) with gradient compression by adding Gaussian noise before quantization, satisfying DP. Lyu et al.~\cite{lyu2021dp} proposed a 1-bit compressor integrating DP into quantization but relies on a fixed quantizer, limiting its adaptability to varying communication budgets. These approaches typically assume a trusted server, unlike LDP, which provides client-side privacy guarantees against potentially curious servers \cite{chaudhuri2022privacy}. While \texttt{FedMPDD} shares the characteristic of achieving both communication efficiency and privacy, our approach differs fundamentally: privacy emerges as a natural consequence of the geometric properties of our communication reduction mechanism, rather than through explicit noise addition or quantization-based schemes.

==> intro2.tex <==
\section{Introduction}\label{sec::Intro}
Federated Learning (FL) is a foundational paradigm for collaboratively training models across $N$ edge devices by leveraging their local computational resources~\cite{mcmahan2017communication, kairouz2021advances, chen2019deep, wang2023model, zeng2021federated}. FL seeks to solve the distributed optimization problem
\begin{equation}\label{eq::opt_prob}
\text{minimize}_{\vect{x}\in\mathbb{R}^d}~~ f(\vect{x}) = \frac{1}{N} \sum\nolimits_{i=1}^N f_i(\vect{x}),
\end{equation}
where $f_i:\mathbb{R}^d\to\mathbb{R}$ is the local objective (loss) function of client $i$, and $f:\mathbb{R}^d\to\mathbb{R}$ is the global objective. Lacking central access to local objectives, FL iteratively communicates between a server and a client subset $\mathcal{A}_k$ ( $|\mathcal{A}_k|=\beta N$, where \( \beta \in (0, 1] \) denotes the client participation rate). In each round $k$, the server sends out the global model $\vect{x}_k$. Selected clients compute local updates (e.g., mini-batch gradients $\vect{g}_i(\vect{x}_k)$) and transmit them to the server. The server aggregates these gradients by averaging: $\vect{g}(\vect{x}_k) = \frac{1}{\beta N} \sum_{i \in \mathcal{A}_k} \vect{g}_i(\vect{x}_k)$, and updates the global model: $\vect{x}_{k+1} = \vect{x}_k - \eta ~\vect{g}(\vect{x}_k)$, as in \texttt{FedSGD}~\cite{mcmahan2017communication}, where $\eta$ is a suitable learning rate.

\medskip

A key bottleneck in FL algorithms like \texttt{FedSGD} is the substantial uplink communication overhead from transmitting $d$-dimensional gradients $\vect{g}_i(\vect{x}_k)$ from clients to the server, requiring \(32d\) bits per client per round, assuming single-precision floating-point representation (32 bits per value). For instance, a ResNet-18 model ($\sim 11 \times 10^6$ parameters) necessitates approximately $42$MB transmission per client per round. This high cost severely impacts efficiency in bandwidth-constrained real-world deployments~\cite{chen2021communication, niknam2020federated, shahid2021communication, li2020federated}. Strategies to reduce FL communication volume or frequency fall into three main classes: \emph{model compression}, \emph{local computation with client selection}, and \emph{gradient compression}. Model compression reduces global model size, for example, by using smaller models with local representations~\cite{liang2020think}. Local computation and client selection decrease communication frequency or the number of clients per round through techniques like multiple local updates~\cite{stich2018local, mcmahan2017communication, karimireddy2020scaffold} and client subset selection~\cite{sattler2019robust, liang2020think}. Gradient compression reduces the size of transmitted gradients using methods like quantization~\cite{alistarh2017qsgd, horvoth2022natural, karimireddy2019error,shlezinger2020uveqfed, bernstein2018signsgd, reisizadeh2020fedpaq, suresh2017distributed}, sparsification~\cite{ivkin2019communication, lin2017deep}, and structured/sketched updates~\cite{konevcny2016federated, wang2020federated, azam2021recycling, han2024random, ivkin2019communication, cho2024heterogeneous, kuo2024federated, qi2024fdlora, yi2023pfedlora, lin2022personalized}. While these existing approaches provide varying degrees of communication reduction, they often face trade-offs between compression ratio, computational overhead, convergence guarantees, and adaptability to different communication budgets, motivating the need for fundamentally new paradigms that can achieve more aggressive communication reduction without sacrificing convergence performance. This paper proposes \texttt{FedMPDD} (\underline{Fed}erated learning with \underline{M}ulti-\underline{P}rojected \underline{D}irectional \underline{D}erivatives), a novel framework that fundamentally tackles the critical communication efficiency bottleneck to enable more practical and scalable deployment of FL in bandwidth-constrained environments. 

\medskip
Unlike existing gradient compression techniques such as quantization, sparsification, or structured/sketched updates, our approach introduces a fundamentally new multiplicative encoding paradigm through the \emph{projected directional derivative} within the FL framework. The method we propose follows the core structure of \texttt{FedSGD} but achieves dramatic communication reduction by employing the \emph{projected directional derivative} $\hat{\vect{g}}_i(\vect{x}_k)=\vect{u}_{k,i}^\top\vect{g}_i(\vect{x}_k)\vect{u}_{k,i}$ (defined in~\eqref{def:proj}) instead of the full stochastic gradient $\vect{g}_i(\vect{x}_k)$. We decompose this projected directional gradient into a scalar directional derivative 
$\vect{u}_{k,i}^\top \vect{g}_i(\vect{x}_k)$ computed locally by client $i$. Each client independently samples $\vect{u}_{k,i}$, then transmits only two scalars: the directional derivative $\vect{u}_{k,i}^\top \vect{g}_i(\vect{x}_k)$ and the random seed $r_{k,i}$ used to generate $\vect{u}_{k,i}$. On the server side, the received seed $r_{k,i}$ is used to reconstruct the identical $d$-dimensional vector $\vect{u}_{k,i}$, enabling the server to form the gradient estimator $\hat{\vect{g}}_{i}(\vect{x}_{k})$ without ever transmitting the full vector. However, our analysis shows that the noisy gradient estimator from a single projected directional derivative would severely degrade performance. To address this, we propose our main algorithm \texttt{FedMPDD}, which introduces a principled multi-projection aggregation mechanism that averages $m$ projected directional derivatives. We show that when $m$ independent projections are aggregated, the classical Johnson--Lindenstrauss guarantees (see details in section \ref{sec::Multi-projection}) ensure that the gradient norm is preserved up to small distortion with high probability. As a result, \texttt{FedMPDD} achieves accurate and stable gradient approximation by transmitting only $m+1$ scalars per client per round---reducing communication from $32d$ to $32(m+1)$ bits and achieving orders of magnitude savings (e.g., from $42$MB to kilobytes for ResNet-18) while maintaining convergence rates comparable to full-gradient methods.


\medskip
While our primary focus is communication efficiency, an interesting and highly valuable emergent property of our encoding scheme is that it naturally provides some level of privacy protection. In FL implementations, Gradient Inversion Attacks (GIAs)~\cite{zhu2019deep, zhao2020idlg, huang2021evaluating, yin2021see, melis2019exploiting, li2022e2egi} remain a critical security concern, where a curious server can reconstruct raw data from transmitted gradients. Conventional defenses, such as Local Differential Privacy (LDP)~\cite{wei2020federated, truex2020ldp, zhao2020local, seif2020wireless}, rely on injecting noise, which introduces a known trade-off between privacy guarantee and model convergence~\cite{jere2020taxonomy}. In stark contrast, the privacy preservation in \texttt{FedMPDD} arises inherently from the geometric properties of our communication reduction mechanism. Specifically, the encoding matrix $\vect{u}_{k, i}\vect{u}_{k, i}^\top$ is rank-deficient ($rank=1 \ll d$), which creates an underdetermined system when attempting to invert the gradient. This nullspace property prevents unique gradient recovery, offering a uniform privacy defense against GIAs that is fundamentally different from additive noise methods and is achieved without sacrificing the communication~benefits. 

\medskip

\subsection{Related Work.} 
The \emph{projected directional derivative} has been explored in optimization, including balancing computational cost and memory in deep learning gradient calculations~\cite{fournier2023can, ren2022scaling, silver2021learning, baydin2022gradients} and in zeroth-order optimization~\cite{nesterov2017random}. To our knowledge, this is the first work to introduce the \emph{projected directional derivative} in FL, specifically through a novel multi-projection decomposition that addresses the dimension-dependent convergence limitations of single-projection methods while achieving substantial communication reduction. 

Our method is fundamentally distinct from structured and sketched updates, which reduce communication by projecting data onto a \textit{fixed}, low-dimensional subspace. Structured updates, such as low-rank adaptation, use a pre-defined subspace for parameters \cite{hu2022lora, yi2023pfedlora, qi2024fdlora, zhang2018systematic, ullrich2017soft, bertsimas2023new, cho2024heterogeneous}. Similarly, sketched updates compress gradients using a shared random matrix, fixed at initialization, via techniques like projection matrices \cite{park2023regulated, azam2021recycling, guo2024low} or Count-Sketch \cite{ivkin2019communication, rothchild2020fetchsgd, haddadpour2020fedsketch, jiang2018sketchml}. These approaches rely on a static projection for all clients and rounds. In contrast, our approach uses a \textit{dynamic} projection strategy based on multi-projected directional derivatives.\margin{I am taking out the next like, I dont think we need it} %We compute $\hat{g}_i(x_k) = (u_{k,i}^\top g_i(x_k)) u_{k,i}$, where the projection directions $u_{k,i}$ are randomly and independently sampled for each client $i$ at every round $k$. 
By averaging multiple projections ($m \ll d$), we overcome the rank-deficiency of a single direction and achieve $O(1/\sqrt{K})$ convergence while reducing communication to $O(m)$ bits. This dynamic multi-projection mechanism simultaneously provides dramatic communication reduction and, as an inherent by-product, privacy protection through the nullspace effect, representing a fundamental departure from methods reliant on fixed subspaces.

Regarding communication efficiency with privacy attributes, other schemes have also shown that communication management can yield privacy benefits \cite{lang2023joint, agarwal2018cpsgd}. For example, Amiri et al.~\cite{amiri2021compressive} combined differential privacy (DP) with gradient compression by adding Gaussian noise before quantization, satisfying DP. Lyu et al.~\cite{lyu2021dp} proposed a 1-bit compressor integrating DP into quantization but relies on a fixed quantizer, limiting its adaptability to varying communication budgets. These approaches typically assume a trusted server, unlike LDP, which provides client-side privacy guarantees against potentially curious servers \cite{chaudhuri2022privacy}. While \texttt{FedMPDD} also achieves both communication efficiency and privacy, our approach differs fundamentally: privacy emerges as a natural consequence of the geometric properties of our communication reduction mechanism, rather than through explicit noise addition or quantization-based schemes.

\subsection{Contribution and the layout of the paper}
The key contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=10pt]
    \item Significant Communication Reduction: \texttt{FedMPDD} dramatically reduces uplink communication from $O(d)$ to just $m + 1$ scalars per client per round ($O(m)$ bits, where $m \ll d$). 

    \item Fast Convergence with Multi-Projection Averaging: Through our novel multi-projection averaging mechanism, \texttt{FedMPDD} achieves a state-of-the-art convergence rate of $O(1/\sqrt{K})$ (Theorem~\ref{thm:main_2}), comparable to the uncompressed \texttt{FedSGD} baseline. The parameter $m$ provides a tunable trade-off between communication cost and convergence speed.
    
    \item Inherent Privacy Preservation: As a natural by-product of our rank-deficient communication scheme, \texttt{FedMPDD} provides an inherent and uniform defense against GIA attacks with limited storage memory without the need for convergence-degrading noise injection.\margin{let's come back to this later}
\end{itemize}

\reza{The remainder of this paper is organized as follows. Section~\ref{sec:mpdd_part} introduces the projected directional derivative, provide the motivation behind the proposed approach, and describe a naive implementation of the proposed mechanism and its challenges. Section~\ref{sec::Multi-projection} then presents the \texttt{FedMPDD} algorithm, details its update steps, and develops the convergence analysis, including convergence rates and privacy-preservation properties. Section~\ref{sec:experiment} reports numerical experiments, and Section~\ref{sec:conclo} concludes the paper.}


Extensive comparative theoretical analysis and empirical evaluations in Sections \ref{sec::Multi-projection} and \ref{sec:experiment}  demonstrate \texttt{FedMPDD}'s superior communication efficiency and model performance, with the added advantage of inherent privacy preservation attributes. Due to space limitations, proofs of some auxiliary lemmas and supplementary experimental results are deferred to the extended arXiv version of this paper~\cite{arxiv_version}.


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> privacy_v0.tex <==
\subsection{Privacy Preservation attributes of \texttt{FedMPDD}} The privacy guarantees of \texttt{FedMPDD} are demonstrated under a standard honest-but-curious threat model, which provides a formal basis for our analysis.

\begin{definition}[\emph{Threat model}]\label{threat_model}\rm{
An \emph{honest-but-curious} adversary (e.g., the server) correctly follows the protocol but attempts to infer private client data by analyzing all accessible information, which includes communication messages, model architecture, and global hyperparameters. }\boxend
\end{definition}

\medskip
Against this adversary, \texttt{FedMPDD}'s privacy stems from its rank-deficient projection ($m \ll d$), which creates a quantifiable uncertainty for any party observing the transmitted data. We formalize this protection below.

\begin{lem}[Gradient reconstruction error]\label{lem:var_estimator_mpdd_final_adjusted}
For the reconstructed gradient estimator $\hat{\vect{g}}_i(\vect{x}_k) = \frac{1}{m} \sum_{j=1}^m \vect{u}^{(j)}_{k,i} (\vect{u}^{(j)}_{k,i})^\top \vect{g}_i(\vect{x}_k)$, the expected relative squared error between the reconstructed and true stochastic gradients is given by:
\begin{equation}\label{eq:relative_error_mpdd_final_adjusted}
\mathbb{E}_{\mathbf{U}} \big[ \| \hat{\vect{g}}_i(\vect{x}_k) - \vect{g}_i(\vect{x}_k) \|^2 \big] \big/ \| \vect{g}_i(\vect{x}_k) \|^2 = \frac{d-1}{m}.
\end{equation}
\boxend
\end{lem}

This inherent gradient ambiguity provides a formal defense against GIAs by establishing a lower bound on an adversary's ability to reconstruct the original private input data.

\begin{lem}[Lower bound on private data reconstruction error, For proof see Appendix \ref{sec:proofs}]\label{lem:feature_recovery_bound}
Suppose an adversary attempts to reconstruct a private input vector $v$ by minimizing the loss between the observed projected gradient and a dummy gradient, $\mathcal{L}(\hat{v}) := \| \tfrac{1}{m} U_{k,i} U_{k,i}^\top \vect{g}_i(v,c;\vect{x}_k) - \vect{g}_i(\hat{v},c;\vect{x}_k) \|$. The expected reconstruction error for the attack-optimal output $\hat{v}^*$ is lower bounded by:
\begin{equation}\label{eq:feature_recovery_bound}
\mathbb{E}\big[ \| v - \hat{v}^* \|^2 \big] \geq \frac{d-1}{m \cdot L_v(\vect{x})^2} \| \vect{g}_i(v,c;\vect{x}_k) \|^2,
\end{equation}
where $L_v(\vect{x})$ is the Lipschitz constant of the gradient with respect to $v$.
\boxend
\end{lem}

\begin{figure}[t]
\centering
    \includegraphics[width=0.43\textwidth]{figs/cropped_k=600_ssim_lenet.png}
    \caption{{\footnotesize The SSIM scores from the GIA~\cite{yu2025gi} on the LeNet model, using the \emph{projected directional derivative} estimator with \( m = 600 \) in \texttt{FedMPDD}, remain consistently low (below 0.04) over 100 training epochs. As showed by Lemma \ref{lem:var_estimator_mpdd_final_adjusted} and \ref{lem:feature_recovery_bound}, this demonstrates that the privacy level remains stable and is independent of the training stage.
}}
\label{fig:ssim_lenet}
\end{figure}


Together, these lemmas establish a direct link between our projection mechanism and a concrete privacy guarantee. The gradient reconstruction error of $\frac{d-1}{m}$ translates into a formal lower bound on data recovery, creating a privacy barrier that scales with model dimension $d$. 
Our approach offers fundamental advantages over additive-noise methods like Local Differential Privacy (LDP). In LDP, the privacy level is inconsistent, as its relative reconstruction error is proportional to $1/\|\vect{g}_i(\vect{x}_k)\|^2$ as shown in Remark~\ref{rem::consistentprive} in Appendix \ref{sec:ldp_Fedmpdd} \margin{I could not find this remark}. This creates a dilemma: large gradients are poorly protected, while small gradients can be overwhelmed by noise, harming model convergence. Achieving consistent privacy with LDP would require large, performance-degrading noise values. In contrast, \texttt{FedMPDD} provides a consistent relative reconstruction error of $\frac{d-1}{m}$, which is independent of the gradient's magnitude. This design simultaneously ensures: (i) consistent privacy without harming utility (by preserving the descent direction), and (ii) high communication efficiency. For a detailed derivation and discussion, please see Appendix~\ref{sec:ldp_Fedmpdd} and \ref{sec:proofs}.



%This approach is fundamentally different from additive-noise methods like Local Differential Privacy (LDP), as our privacy is \emph{consistent} (independent of the gradient's norm), \emph{utility-preserving}, and \emph{communication-efficient}. 

\medskip

Our theoretical guarantees are supported by empirical results. 
For example, Fig.~\ref{cifa10_visul_attack} illustrates the \texttt{FedMPDD} Algorithm's data obfuscation on a client's private data for different values of $m$, as detailed in our numerical examples section. Similar to the observation in Remark~\ref{rem::consistentprive}, \texttt{FedMPDD} inherently provides a consistent relative reconstruction error of $(d-1)/m$ at each communication round. This consistent privacy benefit, independent of gradient size, can be observed in Fig.~\ref{fig:ssim_lenet} in our numerical study (detailed in Appendix \ref{additional_exp}).

% \begin{figure}[t]
% \centering
% \begin{minipage}[t]{0.35\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/visul_ssim_cnn_fedavg_cifar10.png}
%     \label{fig:grad_loss}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.58\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/cifar_10_recunstruct(new).pdf}
% \end{minipage}
% \vspace{-0.1in}
% \caption{ {\footnotesize
% GIA attack \cite{yu2025gi} visualization: SSIM scores (left) and reconstructed CIFAR-10 samples (right) across methods. LDP with small noise (columns 3-4) and QSGD (column 5) show significant data leakage. \texttt{FedMPDD} demonstrates stronger privacy (columns 6 and 7).
% %Visualization of SSIM scores versus the number of iterations during the GIA \cite{zhu2019deep} on the left, and reconstructed CIFAR-10 samples after GIA across various methods on the right. The results demonstrate that the small noise levels used in LDP-based approaches (columns 3 and 4) are insufficient to prevent data leakage. Moreover, as anticipated, the quantization-based method in \cite{alistarh2017qsgd} (column 5) also fails to protect client data, as its primary objective is communication reduction rather than privacy preservation as the reconstructed images still reveal recognizable features of the client’s local data. In contrast, our method \texttt{FedMPDD} achieves significantly lower reconstruction quality for the attacker, indicating stronger privacy preservation.
% }}\vspace{-0.1in}
% \label{cifa10_visul_attack}
% \end{figure}


\begin{figure}[t]
\centering
\begin{minipage}[t]{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/visul_ssim_cnn_fedavg_cifar10.png}
    \label{fig:grad_loss}
\end{minipage}
\hfill
\begin{minipage}[t]{0.58\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/cifar_10_recunstruct(new).pdf}
\end{minipage}

\caption{ {\footnotesize
GIA attack \cite{yu2025gi} visualization: SSIM scores (left) and reconstructed CIFAR-10 samples (right) across methods. LDP with small noise (columns 3-4) and QSGD (column 5) show significant data leakage. \texttt{FedMPDD} demonstrates stronger privacy (columns 6 and 7).
}}
\label{cifa10_visul_attack}
\end{figure}
\begin{remark}[Multi-round privacy composition and adversarial memory models]
\rm{
A key consideration is privacy erosion from an adversary observing a client over multiple rounds. Our formal analysis in Appendix~\ref{sec:multi-round} shows that even in a worst-case scenario (e.g., a static gradient), unique gradient recovery is impossible as long as $T \times m < d$, where $T$ is the number of rounds. This guarantee assumes a \emph{memory-bounded adversary} capable of storing up to $T$ observations—in contrast to standard cryptographic~\cite{dwork2006calibrating} and control-theoretic~\cite{teixeira2015secure} frameworks that often model unbounded-memory adversaries. However, this assumption remains practically relevant: with $d \in [10^6, 10^9]$ parameters and typical training requiring $T \in [10^2, 10^4]$ rounds with $m \ll d$, the condition $T \times m < d$ is easily satisfied (e.g., $d = 10^6$, $m = 100$ allows $T < 10^4$ rounds). Moreover, gradient evolution during training provides additional protection beyond the worst-case static analysis~\cite{geiping2020inverting}. From a control-theoretic perspective, the bound reflects an \emph{observability constraint}: the adversary's rank-$m$ measurement space per round is insufficient to reconstruct the full $d$-dimensional state. Extending guarantees to unbounded-memory adversaries remains important future work.
}
\boxend
\end{remark}

